Anomaly Clustering: Grouping Images into Coherent Clusters of Anomaly Types

We study anomaly clustering, grouping data into coherent clusters of anomaly types. This is different from anomaly detection that aims to divide anomalies from normal data. Unlike object-centered image clustering, anomaly clustering is particularly challenging as anomalous patterns are subtle and local. We present a simple yet effective clustering framework using a patch-based pretrained deep embeddings and off-the-shelf clustering methods. We define a distance function between images, each of which is represented as a bag of embeddings, by the Euclidean distance between weighted averaged embeddings. The weight defines the importance of instances (i.e., patch embeddings) in the bag, which may highlight defective regions. We compute weights in an unsupervised way or in a semi-supervised way when labeled normal data is available. Extensive experimental studies show the effectiveness of the proposed clustering framework along with a novel distance function upon exist-ing multiple instance or deep clustering frameworks. Over-all, our framework achieves 0.451 and 0.674 normalized mutual information scores on MVTec object and texture categories and further improve with a few labeled normal data (0.577, 0.669), far exceeding the baselines (0.244, 0.273) or state-of-the-art deep clustering methods (0.176, 0.277).

==> table/figure_07.tex <==
\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{fig/nmi-vs-labeled-normal.pdf}
    \caption{NMI scores of semi-supervised anomaly clustering with varying ratio of labeled normal data. Plots with dotted line is unsupervised anomaly clustering results with the proposed weighted distance.}
    \label{fig:abl_nmi_vs_labeled_normal}
\end{figure}
\fi

\begin{figure}[t]
    \begin{minipage}[c]{0.6\textwidth}
    \centering
    \includegraphics[width=0.8\linewidth]{fig/nmi-vs-labeled-normal.pdf}
    \end{minipage}
    \begin{minipage}[c]{0.36\textwidth}
    \caption{NMI scores of semi-supervised anomaly clustering with varying ratios of labeled normal data. Plots with dotted line represent unsupervised anomaly clustering results with the proposed weighted distance.}
    \label{fig:abl_nmi_vs_labeled_normal}
    \end{minipage}
\end{figure}


==> table/table_04.tex <==
\iffalse
\begin{table}[ht]
    \centering
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
        \toprule
        Eq.~\eqref{eq:distance_hausdorff_single} & Eq.~\eqref{eq:distance_hausdorff} & Object & Texture & MTD \\
        \midrule
        $\mathrm{mean}$ $\mathrm{mean}$ & -- & 0.166	&	0.162	&	0.058\\
        $\max$ $\min$ & $\max$ & \textbf{0.415}	&	\textbf{0.644}	&	\textbf{0.164} \\
        $\max$ $\min$ & $\mathrm{mean}$ & 0.370	&	0.552	&	0.156\\
        $\min$ $\min$ & -- & 0.105	&	0.183	&	0.127\\
        $\mathrm{mean}$ $\min$ & $\max$ & 0.215	&	0.398	&	0.142\\
        $\mathrm{mean}$ $\min$ & $\mathrm{mean}$ & 0.215	&	0.342	&	0.134\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.05in}
    \caption{NMIs of anomaly clustering using variants of Hausdorff distance. We replace operators in Eq.~\eqref{eq:distance_hausdorff} and \eqref{eq:distance_hausdorff_single} to define variants.}
    \label{tab:exp_variants_hausdorff_dist}
    \vspace{-0.1in}
\end{table}
\fi

% DONE
\begin{table}[ht]
    \centering
    %\resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
        \toprule
        Eq.~\eqref{eq:distance_hausdorff_single} & Eq.~\eqref{eq:distance_hausdorff} & Object & Texture & MTD \\
        \midrule
        %$\mathrm{mean}$ $\mathrm{mean}$ & -- & 0.196 & 0.232 & 0.071 \\
        %$\max$ $\min$ & $\max$ & \textbf{0.415} & \textbf{0.625} & \textbf{0.193} \\
        %$\max$ $\min$ & $\mathrm{mean}$ & 0.372 & 0.562 & 0.160 \\
        %$\min$ $\min$ & -- & 0.126 & 0.187 & 0.130 \\
        %$\mathrm{mean}$ $\min$ & $\max$ & 0.220 & 0.400 & 0.141 \\
        %$\mathrm{mean}$ $\min$ & $\mathrm{mean}$ & 0.235 & 0.348 & 0.134 \\
        $\mathrm{mean}$ $\mathrm{mean}$ & -- & 0.196 & 0.232 & 0.071 \\
        $\max$ $\min$ & $\max$ & \textbf{0.415} & \textbf{0.625} & \textbf{0.193} \\
        $\max$ $\min$ & $\mathrm{mean}$ & 0.372 & 0.562 & 0.160 \\
        $\min$ $\min$ & -- & 0.126 & 0.187 & 0.130 \\
        $\mathrm{mean}$ $\min$ & $\max$ & 0.220 & 0.400 & 0.141 \\
        $\mathrm{mean}$ $\min$ & $\mathrm{mean}$ & 0.235 & 0.348 & 0.134 \\
        \bottomrule
    \end{tabular}
    %}
    \vspace{0.05in}
    \caption{NMIs of anomaly clustering using variants of Hausdorff distance. We replace operators in Eq.~\eqref{eq:distance_hausdorff} and \eqref{eq:distance_hausdorff_single} to define variants.}
    \label{tab:exp_variants_hausdorff_dist}
    \vspace{-0.1in}
\end{table}


==> table/table_05-1.tex <==
\iffalse
% DONE
\begin{table}[t]
    \centering
    %\resizebox{0.92\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
       Variants & Eq.~\eqref{eq:distance_hausdorff_single} & Eq.~\eqref{eq:distance_hausdorff} & Object & Texture & MTD \\
        \midrule
        & $\mathrm{mean}$ $\mathrm{mean}$ & -- & 0.196 & 0.232 & 0.071 \\
        & $\max$ $\min$ & $\max$ & \textbf{0.415} & \textbf{0.625} & \textbf{0.193} \\
       Hausdorff & $\max$ $\min$ & $\mathrm{mean}$ & 0.372 & 0.562 & 0.160 \\
       distance & $\min$ $\min$ & -- & 0.126 & 0.187 & 0.130 \\
        & $\mathrm{mean}$ $\min$ & $\max$ & 0.220 & 0.400 & 0.141 \\
        & $\mathrm{mean}$ $\min$ & $\mathrm{mean}$ & 0.235 & 0.348 & 0.134 \\
        \midrule
        \midrule
        Variants & \multicolumn{2}{c|}{Eq.~\eqref{eq:weighted_distance_unsup}} & Object & Texture & MTD \\
        \midrule
        Unsup. & \multicolumn{2}{c|}{$\mathbb{E}_{j\neq i}$} & 0.451 & \textbf{0.674} & \textbf{0.179} \\
        weights &\multicolumn{2}{c|}{$\max_{j\neq i}$} & 0.252 & 0.614 & 0.138 \\
        &\multicolumn{2}{c|}{$\min_{j\neq i}$} & \textbf{0.472} & 0.625 & 0.052 \\
        \bottomrule
    \end{tabular}
    %}
    \vspace{0.05in}
    \caption{NMIs of anomaly clustering using variants of Hausdorff distance and unsupervised weights. 
    %We replace operators in Eq.~\eqref{eq:distance_hausdorff}, \eqref{eq:distance_hausdorff_single} and~\eqref{eq:weighted_distance_unsup} to define variants.
    }
    \label{tab:exp_variants_dist_measure}
    \vspace{-0.15in}
\end{table}
\fi

% DONE
\begin{table}[t]
    \begin{minipage}{0.55\linewidth}
        \centering
        \resizebox{0.92\linewidth}{!}{%
        \begin{tabular}{c|c|c|c|c|c}
            \toprule
           {  }Variants{  } & {  }Eq.~\eqref{eq:distance_hausdorff_single}{  } & {  }Eq.~\eqref{eq:distance_hausdorff}{  } & {  }Object{  } & {  }Texture{  } & {  }MTD{  } \\
            \midrule
            & {  }$\mathrm{mean}$ $\mathrm{mean}${  } & -- & 0.196 & 0.232 & 0.071 \\
            & $\max$ $\min$ & $\max$ & \textbf{0.415} & \textbf{0.625} & \textbf{0.193} \\
           {  }Hausdorff{  } & $\max$ $\min$ & $\mathrm{mean}$ & 0.372 & 0.562 & 0.160 \\
           {  }distance{  } & $\min$ $\min$ & -- & 0.126 & 0.187 & 0.130 \\
            & $\mathrm{mean}$ $\min$ & $\max$ & 0.220 & 0.400 & 0.141 \\
            & $\mathrm{mean}$ $\min$ & $\mathrm{mean}$ & 0.235 & 0.348 & 0.134 \\
            \midrule
            \midrule
            Variants & \multicolumn{2}{c|}{Eq.~\eqref{eq:weighted_distance_unsup}} & Object & Texture & MTD \\
            \midrule
            {  }Unsup.{  } & \multicolumn{2}{c|}{$\mathbb{E}_{j\neq i}$} & 0.451 & \textbf{0.674} & \textbf{0.179} \\
            {  }weights{  } &\multicolumn{2}{c|}{$\max_{j\neq i}$} & 0.252 & 0.614 & 0.138 \\
            &\multicolumn{2}{c|}{$\min_{j\neq i}$} & \textbf{0.472} & 0.625 & 0.052 \\
            \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \begin{minipage}{0.43\linewidth}
        \caption{NMIs of anomaly clustering using variants of Hausdorff distance and unsupervised weights. 
        %We replace operators in Eq.~\eqref{eq:distance_hausdorff}, \eqref{eq:distance_hausdorff_single} and~\eqref{eq:weighted_distance_unsup} to define variants.
        }
        \label{tab:exp_variants_dist_measure}
    \end{minipage}
    \vspace{-0.15in}
\end{table}


==> table/table_05.tex <==
\iffalse
\begin{table}[ht]
    \centering
    \resizebox{0.62\linewidth}{!}{%
    \begin{tabular}{c|c|c|c}
        \toprule
        Eq.~\eqref{eq:weighted_distance_unsup} & Object & Texture & MTD \\
        \midrule
        $\mathbb{E}_{j\neq i}$ & 0.448 & \textbf{0.666} & \textbf{0.164} \\
        $\max_{j \neq i}$ & 0.250 & 0.649 & 0.142\\
        $\min_{j \neq i}$ & \textbf{0.466} & 0.628 & 0.058\\
        \bottomrule
    \end{tabular}
    }
    \caption{NMIs of anomaly clustering using variants of unsupervised weight. We replace an operator in Eq.~\eqref{eq:weighted_distance_unsup} to define variants.}
    \label{tab:exp_variants_weights}
\end{table}
\fi

% DONE / DONE
\iffalse
\begin{table}[ht]
    \centering
    \resizebox{0.62\linewidth}{!}{%
    \begin{tabular}{c|c|c|c}
        \toprule
        Eq.~\eqref{eq:weighted_distance_unsup} & Object & Texture & MTD \\
        \midrule
        %$\mathbb{E}_{j\neq i}$ & 0.451 & \textbf{0.649} & \textbf{0.179} \\
        %$\max_{j\neq i}$ & 0.209 & 0.647 & 0.138 \\
        %$\min_{j\neq i}$ & \textbf{0.472} & 0.608 & 0.052 \\
        $\mathbb{E}_{j\neq i}$ & 0.451 & \textbf{0.674} & \textbf{0.179} \\
        $\max_{j\neq i}$ & 0.252 & 0.614 & 0.138 \\
        $\min_{j\neq i}$ & \textbf{0.472} & 0.625 & 0.052 \\
        \bottomrule
    \end{tabular}
    }
    \caption{NMIs of anomaly clustering using variants of unsupervised weight. We replace an operator in Eq.~\eqref{eq:weighted_distance_unsup} to define variants.}
    \label{tab:exp_variants_weights}
\end{table}
\fi

\begin{table}[ht]
    \begin{minipage}{0.6\linewidth}
        \centering
        \resizebox{0.95\linewidth}{!}{%
        \begin{tabular}{c|c|c|c}
            \toprule
            Eq.~\eqref{eq:weighted_distance_unsup} & Object & Texture & MTD \\
            \midrule
            %$\mathbb{E}_{j\neq i}$ & 0.451 & \textbf{0.649} & \textbf{0.179} \\
            %$\max_{j\neq i}$ & 0.209 & 0.647 & 0.138 \\
            %$\min_{j\neq i}$ & \textbf{0.472} & 0.608 & 0.052 \\
            $\mathbb{E}_{j\neq i}$ & 0.451 & \textbf{0.674} & \textbf{0.179} \\
            $\max_{j\neq i}$ & 0.252 & 0.614 & 0.138 \\
            $\min_{j\neq i}$ & \textbf{0.472} & 0.625 & 0.052 \\
            \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \begin{minipage}{0.38\linewidth}
        \caption{NMIs of anomaly clustering using variants of unsupervised weight. We replace an operator in Eq.~\eqref{eq:weighted_distance_unsup} to define variants.}
        \label{tab:exp_variants_weights}
    \end{minipage}
\end{table}

==> table/table_06.tex <==
\iffalse
\begin{table}[ht]
    \centering
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{c|c|c|c}
        \toprule
        Dataset & Object & Texture & MTD \\
        \midrule
        WA (Eq.~\eqref{eq:weighted_distance_unsup}) & 0.448 & 0.666 & 0.164 \\
        WA (w/ train) (Eq.~\eqref{eq:weighted_distance_unsup_extra}) & 0.490 & 0.649 & 0.181 \\
        WA (semi) (Eq.~\eqref{eq:weighted_distance_semisup}) & 0.553 & 0.678 & 0.388 \\
        \bottomrule
    \end{tabular}
    }
    \caption{NMIs of weighted average distance based anomaly clustering using different weight computation methods.}
    \label{tab:abl_extra_train_for_weights}
\end{table}
\fi

% DONE / DONE
\begin{table}[ht]
    \centering
    \resizebox{0.4\linewidth}{!}{%
    \begin{tabular}{c|c|c|c}
        \toprule
        Dataset & Object & Texture & MTD \\
        \midrule
        WA (Eq.~\eqref{eq:weighted_distance_unsup}) & 0.451 & 0.674 & 0.179 \\
        WA (w/ train) (Eq.~\eqref{eq:weighted_distance_unsup_extra}) & 0.474 & \textbf{0.676} & {\color{red}0.xxx} \\
        WA (semi) (Eq.~\eqref{eq:weighted_distance_semisup}) & \textbf{0.577} & 0.669 & 0.390 \\
        \bottomrule
    \end{tabular}
    }
    \caption{NMIs of weighted average distance based anomaly clustering using different weight computation methods.}
    \label{tab:abl_extra_train_for_weights}
\end{table}

